Filter-based Discriminative Autoencoders for Children Speech Recognition

Children speech recognition is indispensable but challenging due to the diversity of children's speech. In this paper, we propose a filter-based discriminative autoencoder for acoustic modeling. To filter out the influence of various speaker types and pitches, auxiliary information of the speaker and pitch features is input into the encoder together with the acoustic features to generate phonetic embeddings. In the training phase, the decoder uses the auxiliary information and the phonetic embedding extracted by the encoder to reconstruct the input acoustic features. The autoencoder is trained by simultaneously minimizing the ASR loss and feature reconstruction error. The framework can make the phonetic embedding purer, resulting in more accurate senone (triphone-state) scores. Evaluated on the test set of the CMU Kids corpus, our system achieves a 7.8% relative WER reduction compared to the baseline system. In the domain adaptation experiment, our system also outperforms the baseline system on the British-accent PF-STAR task.

==> rebuttal_0EF3.tex <==
% I have some questions and comments as follows.
% 1) The authors should add "Index Terms".
We will add "Index Terms" in the final paper.

%2) In Section 2.1, the authors should spell out GMM, DNN, HMM, and MMI.
We will spell out GMM, DNN, HMM, and MMI in the final paper.

%3) In Eq. (2), the authors should modify "x" in the denominator to "x_u".
We will correct this error in the final paper.

%4) In Section 3.1, the authors should add a citation to CMU Kids corpus.
We will add the citation in the final paper.

%5) In Section 3.1, the authors should add some explanations to the two children's speech corpora (i.e., CMU Kids corpus and PF-STAR British English children speech corpus), e.g., the range of ages and contents of utterances.
The age range of the CMU Kids corpus is 6-11 years old. The age range of the PF-STAR corpus is 4-14 years old. The speech content mainly consists of reading sentences from sources such as storybooks or textbooks. We will add brief descriptions of these two corpora in the final paper. 

%6) In Section 3.2, the authors should explain why they did not use transcriptions of the two children's speech corpora (i.e., tr_cmu and tr_pfster) for LM training.
We found that the transcriptions of the training and test sets overlap in these two corpora. Therefore, we thought that the transcriptions of training data should not be used to train language models. In [3,4,6], in experiments on the PF-Star corpus, the LM was trained on the WSJ corpus. We followed their experimental setup.

%7) In Section 3.2, the authors should add out-of-vocabulary rates along with the perplexities.
We will provide the out-of-vocabulary rates in the final paper.

%8) In the last sentence of Section 4.1, the authors should modify "8.89%" to "7.00%".
We will correct this error in the final paper.

==> rebuttal_156D.tex <==
%I would suggest one additional reference about the autoencoder-based decomposition strategy, I think it is quite similar to the technique applied here:"Unsupervised Speech Decomposition via Triple Information Bottleneck" by Hasegawa-Johnson et al.

We are grateful for your recommendation and we will cite this paper.

%First, there is a sentence saying "To the best of our knowledge, there is no existing method that can simultaneously optimize the CE, LF-MMI and MSE in acoustic model training". This is definitely perplexing. How the authors trained their model if there is no method to train it using the given loss function? I hope that it is just an incorrectly formulated sentence, and the authors intended to say something else.

We are sorry for the confusion caused by this sentence. We will modify the sentence as "To the best of our knowledge, there is no existing method that simultaneously optimizes the CE, LF-MMI and MSE in acoustic model training." in the final paper.

%We delivered this statement to highlight that training the acoustic model with these 3 types of loss was never proposed in the past until our proposal. There is definitely a method to train it with the given loss. The phrase “there is no existing method” should probably be rephrased to “It is an unprecedented method”, the incorrectly formulated sentence as mentioned in your review.我覺得原句拿掉can似乎就不會引起誤會。

%The other issue is the value of parameter beta, which is the weight of the reconstruction error in the loss function. By setting it to zero, we would go back to the baseline system. However, beta is set to 5x10e-14, which is terribly small, it is hard to believe that it really has an effect on the system. 

The encoder of the f-DcAE acts as the acoustic model of the ASR system. Therefore, its main purpose is to classify the phoneme states of input speech frames. In other words, the loss should strongly consider CE first, followed by LF-MMI that guides the encoder to generate the correct phoneme sequence. If the value of beta (the weight for MSE) is increased, the role of the encoder as a classifier may gradually lose its power and transfer to the role of a generative model, which indirectly harms the output phoneme-states (optimized by CE and LF-MMI).

The adjustment of the value of beta also depends on the size of the corpus. Our acoustic model was trained on the WSJ (adult) and CMU Kids corpora. The adult corpus will inevitably dominate the acoustic model training process because it is much larger than the child corpus. The decoder can be thought of as a regularizer to help the encoder reduce overfitting to adult speech and accommodate child speech more. If the child corpus size gets larger, beta should be even smaller. 

It is also worth mentioning that we use the same beta value for both PF-STAR (British accent) and CMU Kids (American accent) tasks. Experimental results show that the proposed f-DcAE model consistently outperforms the baseline model on both tasks. Even with a small value of beta, the additional MSE loss of the decoder is shown to help improve ASR performance.


==> rebuttal_2B79.tex <==
%Important aspects that are missing:
%- The output label type is not mentioned once and can only be guessed implicitly to be phoneme-related

The output label is the senone (phoneme-state). There are a total of 2,864 senones in this work. We will add a brief description of this in the final paper.

%- The so-called p-code (encoder output) is not sufficiently defined, especially its dimension and definition of corresponding model layer is missing.

In an autoencoder, the output of the encoder is often called the code. It is called the p-code in this work because it contains the phoneme-related information. The p-code is concatenated with the i-vector, the p-vector, or the fusion of the two as the input of the decoder to reconstruct the input acoustic feature. In addition, the p-code is converted into the output scores of senones (phoneme-states) by dense layers. We will add explanations in the final paper.

%- The term p-vector is introduced before properly defining it much later at the end of Sec. 3.1.

The p-vector is defined in [25]. We are sorry we did not cite the reference when the p-vector first appeared in the paper. We will correct this error in the final paper.

%Unclear parts:
%- The beta factor seems unreasonably small, there should be some explanation

The encoder of the f-DcAE acts as the acoustic model of the ASR system. Therefore, its main purpose is to classify the phoneme states of input speech frames. In other words, the loss should strongly consider CE first, followed by LF-MMI that guides the encoder to generate the correct phoneme sequence. If the value of beta (the weight for MSE) is increased, the role of the encoder as a classifier may gradually lose its power and transfer to the role of a generative model, which indirectly harms the output phoneme-states (optimized by CE and LF-MMI).

The adjustment of the value of beta also depends on the size of the corpus. Our acoustic model was trained on the WSJ (adult) and CMU Kids corpora. The adult corpus will inevitably dominate the acoustic model training process because it is much larger than the child corpus. The decoder can be thought of as a regularizer to help the encoder reduce overfitting to adult speech and accommodate child speech more. If the child corpus size gets larger, beta should be even smaller. 

It is also worth mentioning that we use the same beta value for both PF-STAR (British accent) and CMU Kids (American accent) tasks. Experimental results show that the proposed f-DcAE model consistently outperforms the baseline model on both tasks. Even with a small value of beta, the additional MSE loss of the decoder is shown to help improve ASR performance. 

%- Section 3.1: "We raised the pitch of adult speech by setting the parameter pitch [...]": explain what is meant by this.

In this work, We used the sound eXchange toolkit (http://sox.sourceforge.net/sox.html) to raise the pitch of adult test utterances. We will add a brief description of this in the final paper. 

%- What was the speed-perturbation factor in relation to the artificially pitch change of the test sets (if this is what was done)

As is done in most studies, we applied speed perturbation with speed factors of 0.9, 1.0, and 1.1 for data augmentation in training. We used the sound eXchange toolkit (http://sox.sourceforge.net/sox.html) to raise the pitch of adult test utterances to simulate high-pitched speech similar to child speech.

%T. Ko, V. Peddinti, D. Povey, and S. Khudanpur, “Audio augmentation for speech recognition,” in Proc. Interspeech, 2015.
%and will be included in the reference.

%- Lexicon or unknown words are not covered.

We will provide dictionary and out-of-vocabulary (OOV) information in the final paper.

%- i-vector and p-vector only loosely defined, the effect of the 10-frames window is not clear.

In this work, 40-dimensional high-resolution MFCCs were used as the acoustic features. The i-vector was 100-dimensional, extracted every 10 frames, using the built tool in Kaldi. 

The p-vector was 3-dimensional. We computed the pitch mean, the mean delta-pitch, and the normalized cross correlation function (NCCF) of pitches every 10 frames. 

Every 10 frames, each MFCC vector was concatenated with the same i-vector and/or p-vector. For example, the concatenation of MFCCs, i-vector, and p-vector resulted in a 143-dimensional vector. We will add explanations in the final paper.

%We trained a diagonal universal background model (UBM) with 512 Gaussian components based on the 40-dimensional MFCCs of a quarter of the training data to get the i-vector. Principal component analysis (PCA) was used for dimension reduction from 280 (a contextual vector consisting of current, left and right consecutive 3 frames) to 40 before UBM training. The i-vector was extracted every 10 frames. 

 


